Understanding spatial propagation using metric geometry with application to the spread of COVID-19 in the United States

This paper introduces a novel approach to spatio-temporal data analysis using metric geometry to study the propagation of COVID-19 across the United States. Using a geodesic Wasserstein metric, we analyse discrepancies between the density functions of new case counts on any given day, incorporating the geographic spread of cases. First, we apply this to identify the periods during which the changes in the geographic distribution of COVID-19 were most profound. The greatest shift occurred between May and June of 2020, when COVID-19 shifted from mostly dominating the Northeastern states to a wider distribution across the country. We support our findings with a new measure of the extent of geodesic variance of a distribution, demonstrating that the geographic imprint of COVID-19 was most concentrated in May 2020. Next, we investigate whether the epidemic exhibited meaningful patterns of spatial reversion, where similar geographic distributions return later. We identify broad similarity between the spread of COVID-19 across the US between the second and third waves, and to a lesser extent, the reemergence of the first wave's Northeastern dominance closer to the present day. This methodology could provide new insights for analysts to monitor the dynamical spread of epidemics and enable regional policymakers to protect their localities. More broadly, the framework we introduce could be applied to a variety of problems evolving over space and time.

==> Instructions.tex <==
Use eqnarray for multiline equations

\begin{table*}
\caption{\label{tab:table3}This is a wide table that spans the full page
width in a two-column layout. It is formatted using the
\texttt{table*} environment. It also demonstates the use of
\textbackslash\texttt{multicolumn} in rows with entries that span
more than one column.}
\begin{ruledtabular}
\begin{tabular}{ccccc}
 &\multicolumn{2}{c}{$D_{4h}^1$}&\multicolumn{2}{c}{$D_{4h}^5$}\\
 Ion&1st alternative&2nd alternative&lst alternative
&2nd alternative\\ \hline
 K&$(2e)+(2f)$&$(4i)$ &$(2c)+(2d)$&$(4f)$ \\
 Mn&$(2g)$\footnote{The $z$ parameter of these positions is $z\sim\frac{1}{4}$.}
 &$(a)+(b)+(c)+(d)$&$(4e)$&$(2a)+(2b)$\\
 Cl&$(a)+(b)+(c)+(d)$&$(2g)$\footnotemark[1]
 &$(4e)^{\text{a}}$\\
 He&$(8r)^{\text{a}}$&$(4j)^{\text{a}}$&$(4g)^{\text{a}}$\\
 Ag& &$(4k)^{\text{a}}$& &$(4h)^{\text{a}}$\\
\end{tabular}
\end{ruledtabular}
\end{table*}

\begin{table}[b]
\caption{\label{tab:table4}%
Numbers in columns Three--Five are aligned with the ``d'' column specifier 
(requires the \texttt{dcolumn} package). 
Non-numeric entries (those entries without a ``.'') in a ``d'' column are aligned on the decimal point. 
Use the ``D'' specifier for more complex layouts. }
\begin{ruledtabular}
\begin{tabular}{ccddd}
One&Two&
\multicolumn{1}{c}{\textrm{Three}}&
\multicolumn{1}{c}{\textrm{Four}}&
\multicolumn{1}{c}{\textrm{Five}}\\
%\mbox{Three}&\mbox{Four}&\mbox{Five}\\
\hline
one&two&\mbox{three}&\mbox{four}&\mbox{five}\\
He&2& 2.77234 & 45672. & 0.69 \\
C
  &C
  & 12537.64 & 37.66345 & 86.37 \\
\end{tabular}
\end{ruledtabular}
\end{table}


\begin{table}[b]
\caption{\label{tab:table2}
A table with numerous columns that still fits into a single column. 
Here, several entries share the same footnote. 
Inspect the \LaTeX\ input for this table to see exactly how it is done.}
\begin{ruledtabular}
\begin{tabular}{cccccccc}
 &$r_c$ (\AA)&$r_0$ (\AA)&$\kappa r_0$&
 &$r_c$ (\AA) &$r_0$ (\AA)&$\kappa r_0$\\
\hline
Cu& 0.800 & 14.10 & 2.550 &Sn
& 0.680 & 1.870 & 3.700 \\
Ag& 0.990 & 15.90 & 2.710 &Pb
& 0.450 & 1.930 & 3.760 \\
Au& 1.150 & 15.90 & 2.710 &Ca
& 0.750 & 2.170 & 3.560 \\
Mg& 0.490 & 17.60 & 3.200 &Sr
& 0.900 & 2.370 & 3.720 \\
Zn& 0.300 & 15.20 & 2.970 &Li
& 0.380 & 1.730 & 2.830 \\
Cd& 0.530 & 17.10 & 3.160 &Na
& 0.760 & 2.110 & 3.120 \\
Hg& 0.550 & 17.80 & 3.220 &K
&  1.120 & 2.620 & 3.480 \\
Al& 0.230 & 15.80 & 3.240 &Rb
& 1.330 & 2.800 & 3.590 \\
Ga& 0.310 & 16.70 & 3.330 &Cs
& 1.420 & 3.030 & 3.740 \\
In& 0.460 & 18.40 & 3.500 &Ba
& 0.960 & 2.460 & 3.780 \\
Tl& 0.480 & 18.90 & 3.550 & & & & \\
\end{tabular}
\end{ruledtabular}
\end{table}


==> RESPONSE.tex <==
Referee: 1

Referee comments to author(s)
The authors scrutinize spatio-temporal epidemic data by using the geodesic Wasserstein distance metric. This allows for assessing the relationship between the epidemic curves and the geographic spread of cases. This methodology is in the context of theoretical epidemiology novel and leads to important new insights. In the vast majority of recent covid-related studies, the spatial aspect of the epidemic spread was often neglected, even though it represents a very important aspect of this complex process. The findings obtained with this novel theoretical approach are not very surprising, but they are insightful. The framework looks promising, and I think that the manuscript possesses the potential to stimulate further research into spatio-temporal patterns and trends in the disease spread. Therefore, I am in favor of publication of this manuscript. The only minor comment that I have is that the utilization of the geodesic Wasserstein distance might be novel in epidemic research, but it certainly is not a novel metric, as it has been used before to tackle various problems in physics, particularly transport phenomena. This should be briefly discussed in the second chapter of the manuscript.

Thank you for your positive comments on the manuscript and your advice. As suggested, we have edited a paragraph in the second chapter as follows:

``Our primary \st{mathematical} \revision{methodological} contribution is obtained by setting the metric $d$ on $X$ to be the real-world geodesic distances between (the centroids of) the 50 US states and DC, measured in meters. We term the associated Wasserstein distance the \emph{geodesic Wasserstein distance} and notate it as $W_{G}(f,g)$ for two probability vectors $f,g$. \revision{Wasserstein geodesics have been utilised in optimal transport problems \cite{Panaretos2019,Lavenant2019}, but is novel in epidemic research, which frequently neglects the spatial aspect of a virus' spread.}''



Referee: 2

Referee comments to author(s)
Report on the manuscript "Understanding spatial propagation using metric geometry with application to the spread of COVID-19 in the United States" submitted for publication in Europhysics Letters.

In this manuscript, the authors employ the Wasserstein metric to investigate temporal and spatial differences in the PDFs of COVID-19 daily cases for the US states and DC. By using this metric, they are able to identify periods of spatial spread of new cases of the disease. In addition, they are able to verify reversion behaviors where similar patterns appear in different periods of time. The work is interesting and I believe it can be published, but first I wish the authors address some of my concerns.

1) Please include reference regarding COVID-19 vaccination data of US in addition to ref. [2].
https://ourworldindata.org/covid-vaccinations

As suggested, we have added this as a reference in addition to ref. 2.

2) The authors use two Dirac delta functions f and g to show the differences between the discrete and geodesic Wasserstein metric (the latter incorporates the physical distance between the centroid of states/DC into the calculation of the distance). The exposition of this simple case is indeed interesting to visualize the spatial effect in the geodesic variant of the metric. However, I believe a more detailed and marked description of the general case is missing in the text. Although the authors mention that "the geodesic Wasserstein awards a greater distance between two probability vectors if the proportion of cases has shifted further away geographically.", it is not clear that this corresponds to the general case. In addition, the authors could benefit from providing intuition behind the geodesic variant, that is, the geodesic Wasserstein metric can be thought of as the (minimal) cost to transform the distribution of new cases f into g by taking the physical distance into account. Higher values, thus, indicate spatial differences between the distributions f and g as the authors have already pointed out.

As suggested, we have added the following sentences to provide intuition and illustration of the geodesic Wasserstein distance.

``Intuitively, the geodesic Wasserstein metric $W_{G}(f,g)$ is the cost or work (in the sense of physics) to transform the distribution $f$ into $g$, taking real-world distances into account. For example, a shift in distribution from the Northeast to the Appalachian states would be granted a smaller discrepancy difference than a shift from the Northeast to Pacific states.''



3) Table 1 could be replaced by a geographical heatmap (with diverging color palette - https://colorbrewer2.org/#type=diverging) of the values of $\delta(f)_i$ in the main text. A visualization of this type would be more suitable for perceiving spatial shifts in the distribution of daily cases. Table 1 and figure 2 could be moved to supplemental material.

As suggested, we have moved table 1 to the supplementary material, and included a geographical heatmap as a new figure in its place. We have left figure 2 in the manuscript, as we feel it adds additional information beyond the heatmap. The manuscript remains under seven pages. If the editor feels the manuscript is too long, then figure 2 can be moved into the supplementary material as you suggest.

4) Equation (7) expresses a fraction, not a percentage.

We have edited equation (7) to make clear that we multiply by 100 so that the results then described in the table and body of the text are more interpretable.

As suggested, we have edited ``percentage'' to ``fraction.''

5) Figure 4b is missing x, y, and color bar labels. Please include them.

As suggested, we have labelled x and y axes as ``Time'' and color bar ``Geodesic Wasserstein distance.''





6) Overall, the conclusion is confusing. I believe the work would benefit from a thorough revision. 

As suggested, we have carefully revised the conclusion to make it more understandable.

For example, I do not understand what the authors meant to express with this sentence:

(page 5) "June 2020 featured the second wave of COVID-19 in the US as a whole, but the height of the first wave in large states outside the Northeast, such as California, Texas and Florida."

We have edited this sentence (and the one before it) to:

``In May 2020, new COVID-19 cases were mostly concentrated in the Northeastern spread; in June 2020, new cases were spread across the country. During June 2020, the majority of the US was experiencing its second wave of COVID-19; however, California, Texas and Florida, the three largest US states and all outside the Northeast, were experiencing their individual first waves [4].''

Change "lesser" by "a weak":

(page 6) "Lesser similarity is observed between April 2020 and April 2021, signifying a return of the prominence of the Northeastern states."

We have made this change.

Please revise this sentence:

"Studying the time-varying distribution of new COVID-19 cases combined with existing network analyses could provide opportunities for such neighbouring states to work together to combat the ongoing pandemic [37, 38], including against new variants [39] and incorporating the strategic use of vaccinations [40,41]."
suggestion: to work together *combating* the ongoing pandemic [37,38] *and new variants [39],* and incorporating the strategic use of vaccinations [40,41]

Thank you for your attention to detail, we have made this change according to your suggestion and acknowledged your help in the acknowledgments.


Minor:
- (page 1) across US states -> add *and the District of Columbia (DC)*

We have made this change. As this defines the acronym DC earlier, we have edited a later sentence ``let $X$ be the set of the 50 US states and the District of Columbia (DC)'' to ``let $X$ be the set of the 50 US states and DC.''

- (page 2) two probability vectors f, g -> *f and g*

We have made this change.

- (page 2) n = 51 states and DC -> n = 51 *(50 states and DC)*

We have made this change.

- (page 2) index i in equation (2) should begin from 1

I believe you mean equation (5)? Thank you for this correction.

- (page 5) We wish to identify, for some values of t, is there a non-trivial similarity with subsequent times -> *if there is* a non-trivial similarity with subsequent times

We have made this change.

- (page 5) We see two main findings in these figures (With this in mind, two main findings are observed) appears twice

Thank you for this observation, we have removed the first sentence.


- (page 6) if there is *not a* substantial travel between them


Our intention (hypothetically, for future work) is to give a low distance measure between states if there is substantial movement of people (that sort of travel) between them. For substantial travel between states would mean that they could be considered ``close'' (high affinity, low distance) in the sense that case levels could easily spread between the two. We have edited the paragraph to read:

``Future work could modify our framework, replacing geographical distance with other notions of \revision{affinity}. For example, one could consider two locations as \revision{``close''}, and assign them a \revision{high similarity}, if there is \revision{a substantial volume of people travelling} between them. Our methodology could be combined with existing methods of network analysis [36,37] which have also been applied to particular regions [38], or applied on a more granular basis to individual US counties.''


- (page 3 - Sup. Material) exponent 2 in the "y" of equation (17) should not exist

Thank you for this correction.

- (figure 1 caption) proceeding 30 days -> following 30 days

We have made this change.

- include the unit of measure in the x and y labels of plots (m, km, days, etc)

As suggested, we have included units in every x,y label of plots

==> body.tex <==


%Intro to Covid and spatial importance
COVID-19 remains an ongoing threat to the public health of the United States (US). While an aggressive vaccination program has reduced cases and deaths considerably from their highs in January 2021 \cite{vaccinereducedeaths}, the vaccination rate is highly non-uniform across the country \cite{cnnvaxnonuniform}. Communities with low vaccination rates remain a risk, to themselves, as well as to the rest of the nation, both regarding the spread of the virus to vulnerable people elsewhere and the potential for further virus mutation. Throughout the pandemic, the imposition of restrictions on community activity and businesses, including mask mandates and lockdowns, has mostly fallen to state and local governments. Thus, it remains of considerable interest to local lawmakers to track the ongoing spatial propagation of COVID-19 across the US. This may reveal trends in the spread of the virus, allow for forewarning before local outbreaks, identify locations that performed unusually well or poorly in containment measures, and provide opportunities to learn from other localities.


%Prior spatiotemporal or state-by-state
There are numerous existing analyses of the propagation of COVID-19 across the US on a state-by-state or finer basis. Previous research has used a variety of techniques, including state-by-state time series analysis \cite{james2020covidusa,jamescovideu}, SEIR models \cite{Zhou2020_covidUS}, regression models and feature selection \cite{Gross2020,Maiti2021}, Markov chain Monte Carlo models \cite{Paul2020}, and other Monte Carlo simulations \cite{Wang2020_spatioUS}. Similar studies have been carried out in other countries, such as Brazil \cite{Castro2021_Brazil,Ribeiro2020,daSilva2021}, China \cite{Feng2020_spatioChina} and the United Kingdom \cite{Zheng2021}, or comparing numerous countries simultaneously \cite{James2021_virulence,Manchein2020,Jamesfincovid}. Most of these studies are qualitatively descriptive in their summary of the spread of COVID-19 across the geography of a country. 
%Prior physics - maybe new para?
Prior physically-inspired research on COVID-19 has focused on fluids and aerosols \cite{Ng2021_fluids,McRae2021,Verma2020,Yang2020_fluids,Abkarian2020}, characteristics of optimal antigens \cite{Ganti2021},  contagion and percolation models \cite{deArruda2020,Luo2020} and network models \cite{deArruda2020_network, Moore2020, Castellano2020}. Methods from statistical physics have been used widely to study both COVID-19 and prior epidemics \cite{Ganti2021,Silva2019,deArruda2017,Castellano2020}.


%HB: maybe \cal{x}
%where d denotes
%d(x,y) confuse with differential
This paper introduces a new mathematical method for studying the spatial propagation of an epidemic over time. Our approach applies metric geometry to perform an in-depth analysis of the time-varying spatial distribution of COVID-19 cases across US states. Let $(X,d)$ be any metric space, %where $d$ denotes the equipped distance metric,
$\mu,\nu$ two probability measures on $X$, and $q \geq 1$. The Wasserstein metric between $\mu, \nu$ is defined as
\begin{align}
\label{eq:Wasserstein}
    W^q (\mu,\nu) = \inf_{\gamma} \bigg( \int_{X \times X} d(x,y)^q d\gamma  \bigg)^{\frac{1}{q}},
\end{align}
where the infimum is taken over all probability measures $\gamma$ on $X \times X$ with marginal distributions $\mu$ and $\nu$. Henceforth, let $q=1$. By the Kantorovich-Rubinstein formula \cite{Kantorovich}, there is an alternative formulation when X is compact (for example, finite):
\begin{align}
\label{eq:Wassersteinalt}
    W^1 (\mu,\nu) = \sup_{F} \left| \int_{X} F d\mu - \int_{X} F d\nu  \right|,
\end{align}
where the supremum is taken over all $1$-Lipschitz functions $F: X \to \mathbb{R}$. %Further details are provided in supplementary materials.



%Maybe delete "Such probability vectors"
Throughout this paper, let $X$ be the set of the 50 US states and the District of Columbia (DC), ordered alphabetically and indexed $i=1,...,51$. As this is a finite set, measures $\mu,\nu$ may be reinterpreted as probability vectors $f,g \in \mathbb{R}^{51}$ such that $f_i\geq 0$ and $\sum_{i=1}^{51} f_i=1$. Such probability vectors are our central object of study, as they define the spatial distribution over the US. The simplest metric we can equip $X$ with is the discrete metric, where $d(x,y)=1$ if $x\neq y$, and 0 otherwise. In this case, the formulation (\ref{eq:Wassersteinalt}) of Wasserstein metric is optimized with the choice of function
\begin{align}
\label{eq:bestF}
F(x) = \begin{cases}
1, & f(x) \geq g(x), \\
0, & f(x)<g(x), 
\end{cases}
\end{align}
and thus greatly simplifies to a relatively simple metric
\begin{align}
\label{eq:discreteWass}
     W_{disc}(f,g)=\frac12 ||f - g||_1.
\end{align}
A proof of this statement is included in the supplemental material (Proposition 1). We refer to this as the \emph{discrete Wasserstein distance} - it will not be our primary object of study but will be utilized later to demonstrate the robustness of our results.

Our primary mathematical contribution is obtained by setting the metric $d$ on $X$ to be the real-world geodesic distances between (the centroids of) the 50 US states and DC, measured in meters. We term the associated Wasserstein distance the \emph{geodesic Wasserstein distance} and notate it as $W_{G}(f,g)$ for two probability vectors $f,g$.

Consider the illustrative case where $f$ and $g$ are Dirac delta functions supported on single elements $x$ and $y$, respectively. By the formulation (\ref{eq:Wassersteinalt}), it follows that $W^1(f,g)=d(x,y)$. For the discrete Wasserstein distance, this means that $W_{disc}(f,g)=1$ if $x\neq y$, whereas $W_{G}(f,g)$ is the physical distance between (the centroids of the) states indexed by $x$ and $y$. Thus, the geodesic Wasserstein distance allows us to factor in the physical spread of COVID-19 across the US. That is, the discrete Wasserstein distance (or $L^1$ norm) between probability vectors does not take into account distance between states; the geodesic Wasserstein awards a greater distance between two probability vectors if the proportion of cases has shifted further away geographically.

We use this new metric for two aims. First, we wish to determine the periods with the most rapid change in spatial propagation of COVID-19 across the US. Second, we investigate whether there is any reversion behavior in this spatial propagation. While existing studies have typically analyzed the behavior of the different waves of the pandemic on a state-by-state basis, our approach will identify distinct times where a similar geographic distribution of COVID-19 returned across the US. In doing so, it can identify similarities in successive waves of the pandemic.


%However, we exclude the first 50 days of data, in which the daily and 30-day-grouped probability vectors are changing rapidly due to sparsely reported new case counts.
Our data spans March 12, 2020 to June 30, 2021  across $n=51$ states and DC, a period of $T=476$ days. We begin here to avoid periods of sparse reporting early in the pandemic. Our analysis includes Alaska and Hawaii - due to their small contribution to total US case counts, their exclusion has a minimal impact on results. In order to reduce irregularities in daily counts, such as lower reporting of tests on weekends, we first apply a simple 7-day smoothing operator to the counts. This yields a multivariate time series of smoothed new cases $x_i(t), i=1,...,n, t=1,..,T$.  For the first experiment, we consider grouped probability vectors of 30-day periods. Specifically, let $f^{[a:b]}$ be the probability vector of (smoothed) new cases in each state, observed across an interval $a\leq t \leq b$, divided by the total number of US cases across this period:
\begin{align}
f^{[a:b]}_i = \dfrac{\sum_{t=a}^b x_i(t)}{\sum_{t=a}^b \sum_{j=0}^{n} x_j(t)}, i=0,...,n. 
\end{align}
When $a=b$, we simply notate this as $f_i(t)$. In Figure \ref{fig:GW_CPD}, we display the distance function 
\begin{align}
\label{eq:distancefn1}
   t \mapsto W_G(f^{[t-30:t-1]}, f^{[t:t+29]}), \hspace{1em} 31 \leq t \leq T - 29,
\end{align}
 between adjacent 30-day periods. For example, $t=51$ corresponds to May 1, and the associated function value is the geodesic Wasserstein distance between the probability vector of cases across April 1-30 and May 1-30. Within this figure, we also notate local maxima (over a 30-day window). 

The primary finding of this figure is a drastic peak on June 6, 2020. This reveals that the spatial distribution of cases throughout the month of May (broadly speaking) was significantly different to that throughout the month of June. Other more moderate peaks are observed on August 23, 2020,  December 6, 2020, March 5, 2021, and May 30, 2021. Throughout the figure, the function (\ref{eq:distancefn1}) displays approximately periodic intervals of increase and decrease. To complement our primary finding, we take a deeper analysis of the 30-day periods prior to and following our peak date, June 6, 2020.

%NOTE: Throughout the figure, the function (\ref{eq:distancefn1}) consistently displays rather regular patterns of increase and decrease.

%September 9, 2020

The primary difference between the spatial distribution of COVID-19 cases across the US during the months of May and June 2020 is that May was dominated by high numbers of new cases in the Northeastern states, while cases spread much wider in June, impacting larger states such as California, Texas and Florida with significant case counts. We elucidate and quantify this with an individual state-by-state analysis of the distributional changes between May and June.

In Figure \ref{fig:State_density_time_series}, we plot the time-varying probability densities $f_i(t)$ for select states over the period May 7, 2020 to July 5, 2020. These figures show the substantial change in the distribution of COVID-19 across the country during this 60-day period. In Figures \ref{fig:NewYork}, \ref{fig:NewJersey}, \ref{fig:Massachusetts}, \ref{fig:Pennsylvania} respectively, we see that four Northeastern states, New York, New Jersey, Massachusetts, and Pennsylvania exhibit a considerable decline in this period in their proportion of the total new COVID-19 cases across the US. While not a Northeastern state, the similarly urbanized and politically inclined state of Illinois (\ref{fig:Illinois}) also exhibits a drastic decline. On the other hand, California (\ref{fig:California}), Texas (\ref{fig:Texas}), Florida (\ref{fig:Florida}) and Arizona (\ref{fig:Arizona}) exhibit a considerable increase. Altogether, Figure \ref{fig:State_density_time_series} shows the decline in the densities in the Northeastern states and the relative increase in all other areas of the country in the month of June.


%NOTE: converted into a percentage
We provide more quantitative detail in Table \ref{tab:State_density_deltas}, where we compute normalized integrals of the time-varying daily density function $f_i(t)$ for each state between May 7 to June 5 and June 6 to July 5. That is, we compute the following for each state, expressed as a percentage:
\begin{align}
\label{eq:delta_i}
\Delta(f)_i =  \frac{1}{30} \sum_{t=t_0}^{t_0 +29} f_i(t) - \frac{1}{30}\sum_{t=t_0 - 30}^{t_0 - 1} f_i(t).
\end{align}
The states with the largest absolute changes in their average percentage of US total new cases are Florida (increase of 7.59), Texas (increase of 6.25), Illinois (decrease of 6.08), New York (decrease of 5.42), Arizona (increase of 5.00), California (increase of 4.57), New Jersey and Massachusetts (decreases of 3.53 and 3.48 respectively). Across all states, the sum of the absolute value of the changes in average proportion is 67.86\%. As this coincides with an $L^1$ norm between distributions, we deduce that $W_{disc}(f^{[t_0 - 30: t_0 -1]},f^{[t_0: t_0 +29]}) = 0.3393$, by (\ref{eq:discreteWass}). This is a substantial difference (its maximal possible difference is 1), and validates the sizeable change in the distribution of cases between these two 30-day periods.



%HB: I am not sure about the use of the terms spread here (potential confusion with spread of the virus) and also the use of the term variance of a distribution, as the variance of a distribution has a previous definition. Maybe something like "concentration", or lack thereof. But not sure the best term at the moment.
We complete this first analysis with a novel mathematical approach to quantify the spread of a probability distribution across a metric space, while taking the spatial structure into account. Given a distribution $f$ corresponding to a measure $\mu$ on a finite metric space $(X,d)$, let
\begin{align}
\label{eq:geodesicvariance}
\text{Var}(f) = \int_{X \times X} d(x,y)^2 d\mu(x) d\mu(y) = \sum_{x, y \in X} d(x,y)^2 f(x)f(y),    
\end{align}
where the second equality is valid when the metric space is discrete, as in this example. We term (\ref{eq:geodesicvariance}) the \emph{geodesic variance} of the distribution $f$. We explain how this is a generalization of the classic notion of variance in the supplemental material (Proposition 2).

The geodesic variance is zero for a Dirac delta $f=\delta_x$, and greater when the distribution is more spread out across the space. In Figure \ref{fig:GW_Var30}, we plot the time-varying variance of grouped 30-day distributions, $t \mapsto \text{Var}(f^{[t: t+29]})$. This figure reveals that the geographic variance of COVID-19 across the US is globally minimal when $t$ corresponds to May 3, 2020, reflecting the 30-day period until June 1, 2020. From this point, it sharply increases, corresponding to the spread of the virus across the country, complementing the findings already observed.






% \begin{figure*}
%     \centering
%     \includegraphics[width=0.95\textwidth]{Images/d(t,t+1)_geodesic_wasserstein.png}
%     \caption{Sequential geodesic Wasserstein distances. There is a notable peak at June 1 2020, where the dynamics appear to change. Beyond this point, amplitude of $d(t,t+1)$ is larger. Other notable peak at beginning of September 2020.}
%     \label{fig:GW_dt_t+1}
% \end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{Images/GW_CPD_Window.png}
    \caption{Time-varying geodesic Wasserstein distance (in meters) between adjacent aggregated 30-day distributions of new cases. Large spikes in this distance indicate meaningful shifts in the spatial distribution of COVID-19 over a one-two month transition. The large first peak corresponds to June 6, 2020, signifying that the prior and proceeding 30-day periods have substantially different spatial distributions. The prior 30 days (May 7 to June 5) are characterized by the dominance of Northeastern states, while the proceeding 30 days (June 6 to July 5) are characterized by the ascent of case numbers elsewhere, including California, Texas, Florida and Arizona.}
    \label{fig:GW_CPD}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_New York_time_evolving_density.png}
        \caption{}
        \label{fig:NewYork}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_New Jersey_time_evolving_density.png}
        \caption{}
        \label{fig:NewJersey}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_Massachusetts_time_evolving_density.png}
        \caption{}
        \label{fig:Massachusetts}
    \end{subfigure}
    % \begin{subfigure}[b]{0.32\textwidth}
    %     \includegraphics[width=\textwidth]{Individual_states/USA_Connecticut_time_evolving_density.png}
    %     \caption{}
    %     \label{fig:Connecticut}
    % \end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_Pennsylvania_time_evolving_density.png}
        \caption{}
        \label{fig:Pennsylvania}
    \end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_Illinois_time_evolving_density.png}
        \caption{}
        \label{fig:Illinois}
    \end{subfigure}    
% \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{Individual_states/USA_Georgia_time_evolving_density.png}
%         \caption{}
%         \label{fig:Georgia}
%     \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_California_time_evolving_density.png}
        \caption{}
        \label{fig:California}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_Texas_time_evolving_density.png}
        \caption{}
        \label{fig:Texas}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_Florida_time_evolving_density.png}
        \caption{}
        \label{fig:Florida}
    \end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Individual_states/USA_Arizona_time_evolving_density.png}
        \caption{}
        \label{fig:Arizona}
    \end{subfigure}
    \caption{Time-varying densities of new cases for (a) New York (b) New Jersey (c) Massachusetts (d) Pennsylvania (e) Illinois (f) California (g) Texas (h) Florida (i) Arizona across the period May 7 to July 5, 2020. This 60-day interval was identified in Figure \ref{fig:GW_CPD} as the most substantial period of geographic change in the entire period.}
    \label{fig:State_density_time_series}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{Images/Geodesic_variance_grouped_PDF.png}
    \caption{Time-varying geodesic variance (in square meters) (\ref{eq:geodesicvariance}) of 30-day aggregated distributions. The global minimum at May 3, 2020 reflects the spatial concentration of new COVID-19 cases in the Northeastern states during the period May 3 to June 1. In the proceeding 30 days, the geodesic variance grows considerably as new cases become much more spread across the US.}
    \label{fig:GW_Var30}
\end{figure*}





% \begin{enumerate}
%     % \item $d(t,t+1)$ plot - reveal small peak early June, others later.
%     % \item Rolling 30-day window plot, maximum at June 6.
%     % \item More granular look at NY, CA/TX/FL, AZ, with ``integral changes" ie discrete Wasserstein.
%     %\item Table of values with sum 68\%. Normalise by population.
%     %\item $d(s,t)$ plot with the minimum - June 2020 to Jan 2021. June 2020 is US overall 2nd wave but 1st for CA/TX/FL, Jan 2021 is US overall 3rd wave but 2nd for CA/TX/FL.
%     %\item Monotonic tests - little bump?  ``Essentially non-increasing."
% \end{enumerate}


\begin{table}
\begin{center}
\begin{tabular}{ |p{4cm}|p{1.5cm}||p{4cm}|p{1.5cm}|}
%  \hline
%  \multicolumn{4}{|c|}{Country and June-July density changes} \\
 \hline
 State & $\Delta(f)_i $ & State & $\Delta(f)_i $ \\
 \hline
 Alabama & 0.82 & Montana & 0.04 \\
 Alaska & 0.06 & Nebraska & -0.70 \\
 Arizona & 5.00 & Nevada & 0.62 \\
 Arkansas & 0.93 & New Hampshire & -0.19 \\
 California & 4.57 & New Jersey & -3.53 \\
 Colorado & -0.75 & New Mexico & -0.09 \\
 Connecticut & -1.41 & New York & -5.42 \\
 Delaware & -0.41 & North Carolina & 1.58 \\
 District of Columbia & -0.38 & North Dakota & -0.10 \\
 Florida & 7.59 & Ohio & -0.51 \\
 Georgia & 1.09 & Oklahoma & 0.42 \\
 Hawaii & 0.03 & Oregon & 0.30 \\
 Idaho & 0.22 & Pennsylvania & -1.89 \\
 Illinois & -6.08 & Rhode Island & -0.58 \\
 Indiana & -0.94 & South Carolina & 1.96 \\
 Iowa & -0.46 & South Dakota & -0.15 \\
 Kansas & -0.17 & Tennessee & 0.62 \\
 Kentucky & -0.04 & Texas & 6.25 \\
 Louisiana & 0.59 & Utah & 0.70 \\
 Maine & -0.07 & Vermont & 0.01 \\
 Maryland & -2.53 & Virginia & -1.91 \\
 Massachusetts & -3.48 & Washington & 0.23 \\
 Michigan & -0.65 & West Virginia & -0.02 \\
 Minnesota & -1.36 & Wisconsin & -0.09 \\
 Mississippi & 0.13 & Wyoming & 0.02 \\
 Missouri & 0.24 & & \\
\hline
\end{tabular}
\caption{US states and their values of $\Delta(f)_i$, defined in (\ref{eq:delta_i}), measuring the percentage change in their contribution to new US cases between the adjacent 30-day periods of May 7 to June 5 and June 6 to July 5, 2020.}

%We provide more quantitative detail in Table \ref{tab:State_density_deltas}, where we compute normalized integrals of the time-varying daily density function $f_i(t)$ for each state between May 7 to June 5 and June 6 to July 5. That is, we compute the following for each state, expressed as a percentage:
%\label{eq:delta_i}
\label{tab:State_density_deltas}
\end{center}
\end{table}

For our second aim, we investigate the extent of spatial reversion over time. We wish to identify, for some values of $t$, is there a non-trivial similarity with subsequent times $s>t$. For each $t$, we consider intervals $\{s: s \geq t+30 \}$ to avoid trivial similarity with neighbouring times and record both $\min \{W_G(f^{[s:s+29]},f^{[t:t+29]}): s \geq t+30 \}$ and $\argmin \{W_G(f^{[s:s+29]},f^{[t:t+29]}): s \geq t+30 \}$. Ignoring the trivial region of being within 30 days of $t$, these determine the time $s$ whose COVID-19 distribution is most similar to time $t$ as well as the magnitude of that similarity. We plot both the argmin function, in days, and the min function, in meters, in Figure \ref{fig:GW_Spatial_evolution}. To provide more details, we also plot $W_G(f^{[s:s+29]},f^{[t:t+29]})$ for all non-trivial values of $s \geq t+30$ in Figure \ref{fig:GW_min_distance}.



We see two main findings in these figures. In Figure \ref{fig:GW_Spatial_evolution}, non-trivial spatial reversion is characterized by the argmin function being greater than 30 (the nearest permissible day under consideration). With this in mind, two main findings are observed. First, April 2020 has both a high min and argmin, seen in Figure \ref{fig:GW_Spatial_evolution}. The value of the argmin is 350 days, revealing maximal proximity to a period about one year later; the value of the min is approximately 400 km. Thus, this period is not very similar to any other period, but it is weakly similar to April 2021. April 2020 is characterized by the early dominance of the Northeastern US states. This reflects that this period was quite distinct from any other time, but that April 2021 reflects a weak reemergence of the Northeast as significant contributor to the nation's cases.

Secondly, June 2020 is characterized by a relatively low value in the minimum, revealing substantial non-trivial similarity to a subsequent period. The argmin here is approximately 200 days and then immediately after about 360 days. This reflects that June 2020 is highly similar to the period comprising December 2020 and January 2021, as well as the period of June 2021. Indeed, June 2020 is characterized by the second wave of COVID-19 in the US overall, and the first wave in large states California, Texas and Florida, while the beginning of 2021 is characterized by the third wave of COVID-19 in the US overall, and the second wave in the aforementioned large states. The sudden increase in the argmin function around this date reveals additional similarity with June 2021, in which a fourth wave of COVID-19 in the US is beginning. That is, the argmin values around June 2020 reveal two different subsequent reversions in the geographic distribution of COVID-19. This strong similarity is also visible in the darker regions of Figure \ref{fig:GW_min_distance}, to the right of the $y$-value of $t$ as June 1, 2020.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.74\textwidth}
        \includegraphics[width=\textwidth]{Images/GW_Spatial_Evolution_grouped.png}
        \caption{}
        \label{fig:GW_Spatial_evolution}
    \end{subfigure}
    \begin{subfigure}[b]{0.74\textwidth}
        \includegraphics[width=\textwidth]{Images/GW_min_distance_evolution_grouped.png}
        \caption{}
        \label{fig:GW_min_distance}
    \end{subfigure}
    \caption{Spatial reversion of the distribution of COVID-19 cases over time. In (a), we plot both the argmin, in days, and the size of the minimal value, in meters, of $\{W_G(f^{[s:s+29]}, f^{[t:t+29]}): s \geq t+30 \}$ as $t$ varies. Periods where the argmin is greater than 30 indicates non-trivial spatial reversion occurs at a time later than $t$. April 2020 is revealed to be weakly similar to a year in the future, but not to any other time. June 2020 is revealed to be similar to both January 2021 and June 2021. In (b), we plot $W_G(f^{[s:s+29]}, f^{[t:t+29]})$ for all non-trivial values $s \geq t+30$. Substantial similarity between June 2020 and various later times are visible in the darker band to the top right of the figure.}
    \label{fig:SpatialEvolutionDensity}
\end{figure*}

In conclusion, we have introduced a new methodological framework to analyze the spatio-temporal propagation of a process, such as an epidemic across a physical region. Future work could modify our framework, replacing geographical distance with other notions of proximity. For example, one could consider two locations as close, assigning them a low measure of distance, if there is substantial travel between them. Our methodology could be combined with existing methods of network analysis \cite{Hncean2020}, or applied on a more granular basis to individual US counties.

COVID-19 data is sourced from the New York Times \cite{datasourcenyt} and US location data is sourced from Google \cite{datasourceUSgeography}.

% \begin{acknowledgments}
% Acknowledgments here if necessary.
% \end{acknowledgments}

%\appendix
% \appendix %for one appendix

% \section{Appendix \label{appendix}}

% \begin{prop}
% Let $(X,d)$ be a finite discrete metric space, with $d(x,y)=1$ for all $x\neq y$ and zero otherwise. Let $W^1(\mu,\nu)$ be the $L^1$-Wasserstein metric between two probability measures $\mu,\nu$ on $X$, with corresponding distribution functions $f,g$, expressed as in (\ref{eq:Wassersteinalt}). That is,
% \begin{align}
% \label{eq:Wassersteinalt_new}
%     W^1 (\mu,\nu) = \sup_{F} \left| \int_{X} F d\mu - \int_{X} F d\nu  \right|.
% \end{align}
% Then, this supremum is optimized by the choice of $F$ as in (\ref{eq:bestF}), namely
% \begin{align}
% \label{eq:bestF_new}
% F(x) = \begin{cases}
% 1, & f(x) \geq g(x), \\
% 0, & f(x)<g(x).
% \end{cases}
% \end{align}
% As such, $W^1(f,g)$ reduces to the simple form of (\ref{eq:discreteWass}), namely
% \begin{align}
% \label{eq:discreteWass_new}
% W^1(f,g)=\frac12 ||f - g||_1.
% \end{align}
% \end{prop}
% \begin{proof}
% Let $F$ be an arbitrary $1$-Lipschitz function on $X$. That is, $F: X \to \mathbb{R}$ and $|F(x) - F(y)| \leq d(x,y) =1$ for $x\neq y$. Let $M=\sup_{x\in X} F(x), m= \inf_{y \in X} F(y).$ By taking the supremum over $x$ and the infimum over $y$, the Lipschitz condition ensures that $M-m\leq 1.$ So
% \begin{align}
%   \int_{X} F d\mu - \int_{X} F d\nu  &=\sum_{x \in X} F(x)(f(x)-g(x)) \\ &\leq \sum_{x: f(x) \geq g(x) } M(f(x)-g(x)) + \sum_{x: f(x) < g(x) } m(f(x)-g(x))\\
%   &\leq \sum_{x: f(x) \geq g(x) } (m+1)(f(x)-g(x)) + \sum_{x: f(x) < g(x) } m(f(x)-g(x))\\
%   &=\sum_{x: f(x) \geq g(x) } f(x)-g(x) + \sum_{x \in X}m(f(x)-g(x))\\
%   &=\sum_{x: f(x) \geq g(x) } f(x)-g(x),
% \end{align}
% using the fact that $\sum_x f(x)=\sum_x g(x)=1$ to eliminate the second sum. Now, let
% \begin{align}
%     P&=\sum_{x: f(x) \geq g(x) } f(x)-g(x),\\
%     N&=\sum_{x: f(x) < g(x) } g(x)-f(x).
% \end{align}
% Then $P-N = \sum_{x\in X} f(x)-g(x) = 0,$ while $P+N = \sum_{x \in X} |f(x)-g(x)|=\|f-g\|_1.$ Thus, we deduce $P=N=\frac12 \|f-g\|_1,$ and $\left|\int_{X} F d\mu - \int_{X} F d\nu\right| \leq P$. Taking the supremum over $F$, we deduce $W^1(f,g) \leq P$. Finally, let $F$ be as in (\ref{eq:bestF_new}). Then $\int_{X} F d\mu - \int_{X} F d\nu$ immediately coincides with $P$, by definition. Thus, the supremal value coincides with $P$, and $P=\frac12 \|f-g\|_1$, as required.


% \end{proof}

% \begin{prop}
% Let $f$ be a probability distribution on a finite metric space $(X,d)$, and consider its geodesic variance, defined by (\ref{eq:geodesicvariance}). That is,
% \begin{align}
% \label{eq:geodesicvariance_new}
% \text{Var}(f) = \int_{X \times X} d(x,y)^2 d\mu(x) d\mu(y) = \sum_{x, y \in X} d(x,y)^2 f(x)f(y).  
% \end{align}
% When $(X,d)$ is a finite subset of the real numbers $\mathbb{R}$ with its Euclidean metric, this quantity reduces to the classical notion of variance, up to a factor of 2.
% \end{prop}
% \begin{proof}
% Let $Y$ be a random variable on $\mathbb{R}$. The classical notion of variance is the quantity $\text{var}(Y)=\E Y^2 - (\E Y)^2$. If $Y$ has a distribution $f$ over a finite set $X$, this can be expressed
% \begin{align}
%     \text{var}(Y) = \sum_{x \in X} x^2 f(x) - \left(\sum_{x \in X} x f(x)\right)^2.
% \end{align}
% On the other hand, (\ref{eq:geodesicvariance_new}) can be expanded
% \begin{align}
%     \text{Var}(f) &= \sum_{x, y \in X} (x-y)^2 f(x)f(y)\\
%     &=\sum_{x, y \in X} x^2 f(x)f(y) + \sum_{x, y \in X} y^2 f(x)f(y) - 2\sum_{x, y \in X} xyf(x)f(y)\\
%     & = 2\sum_{x, y \in X} x^2 f(x)f(y) - 2\sum_{x, y \in X} xyf(x)f(y)\\
%     &=2\sum_{x \in X} x^2 f(x) - 2 \left(\sum_{x \in X} x f(x)\right)\left(\sum_{y \in X} y^2 f(y)\right)\\
%     &=2\text{var}(Y).
% \end{align}
% Thus, up to a factor of 2, the geodesic variance reduces to the classical notion of variance on the real line. 
% \end{proof}

% With more care, the above propositions hold if $X$ is an arbitrary metric space, with $\mu, \nu$ appropriately integrable measures on $X$.

\bibliography{_references}
\bibliographystyle{apsrev4-2.bst}
\end{document}
